Solid-Fluid Interaction with Surface-Tension-Dominant Contact

We propose a novel three-way coupling method to model the contact interaction between solid and fluid driven by strong surface tension. At the heart of our physical model is a thin liquid membrane that simultaneously couples to both the liquid volume and the rigid objects, facilitating accurate momentum transfer, collision processing, and surface tension calculation. This model is implemented numerically under a hybrid Eulerian-Lagrangian framework where the membrane is modelled as a simplicial mesh and the liquid volume is simulated on a background Cartesian grid. We devise a monolithic solver to solve the interactions among the three systems of liquid, solid, and membrane. We demonstrate the efficacy of our method through an array of rigid-fluid contact simulations dominated by strong surface tension, which enables the faithful modeling of a host of new surface-tension-dominant phenomena including: objects with higher density than water can keep afloat on top of it; 'Cheerios effect' about floating objects that do not normally float attract one another; surface tension weakening effect caused by surface-active constituents.

==> Figures/pushpin.tex <==
\begin{figure*}[t]
    \newcommand{\formattedgraphics}[1]{\includegraphics[width=0.24\textwidth,trim= 0 0 0 0,clip]{#1}}
    \centering
    \formattedgraphics{Figures/pushpin/pushpin_collide0000.jpg}
    \formattedgraphics{Figures/pushpin/pushpin_collide0015.jpg}
    \formattedgraphics{Figures/pushpin/pushpin_collide0107.jpg}
    \formattedgraphics{Figures/pushpin/pushpin_collide0150.jpg}
    \\
    \formattedgraphics{Figures/pushpin/output_sink_mesh0000.jpg}
    \formattedgraphics{Figures/pushpin/output_sink_mesh0060.jpg}
    \formattedgraphics{Figures/pushpin/output_sink_mesh0074.jpg}
    \formattedgraphics{Figures/pushpin/output_sink_mesh0093.jpg}
    \caption{Push Pin}
    \label{fig:pushpin}
\end{figure*}

==> Figures/teaser.tex <==
% A "teaser" figure, centered below the title and authors and above the body of the work.
\begin{teaserfigure}
  \centering
  \includegraphics[width=\linewidth]{Figures/Teaser2.png}
  \caption{Teaser Figure Here}
\end{teaserfigure}

==> bo_notes.tex <==
Cheerios effect:
https://en.wikipedia.org/wiki/Cheerios_effect#:~:text=In%20fluid%20mechanics%2C%20the%20Cheerios,normally%20float%20attract%20one%20another.&text=It%20is%20named%20after%20the,the%20surface%20of%20soft%20drinks.

https://www.nbcnews.com/id/wbna9425907

Bush's notes:
Asweshall soon see, surface tensiondominatesgravity ona scaleless thanthe capillary length(roughly 2mm). It thus plays a critical role in a variety of small-scale processes arising in biology, environmental science and technology.


Asweshall soon see, surface tensiondominatesgravity ona scaleless thanthe capillary length(roughly 2mm). It thus plays a critical role in a variety of small-scale processes arising in biology, environmental science and technology.
Biology
•
all small creatures live in a world dominated by surface tension
•
surface tension important for insects for many basic functions
•
weight support and propulsion at the water surface
•
adhesion and deadhesion via surface tension
•
the pistol shrimp: hunting with bubbles
•
underwater breathing and diving via surface tension
•
natural strategies for water-repellency in plants and animals
•
the dynamics of lungs and the role of surfactants and impurities
Figure 2.1: The diving bell spider
Geophysics and environmental science
•
thedynamicsofraindrops andtheirroleinthe biosphere
•
mostbiomaterialis surface active, stickstothe surface ofdrops/ bubbles
•
chemical, thermal and biological transport in the surf zone
•
early life: early vessicle formation, confinement to an interface
• oil recovery, carbon sequestration, groundwater flows
•
design of insecticides intended to coat insects, leave plant unharmed
•
chemical leaching and the water-repellency of soils
• oil spill dynamics and mitigation
•
disease transmission via droplet exhalation
•
dynamics of magma chambers and volcanoes
•
the exploding lakes of Cameroon
Technology
•

%%%% intro
%% Big picture
%% 讲一下物理原理，画一个示意图
%Accurate contact modeling between solid and fluid is essential for physics simulation on a microscopic level (between millimeter to centimeters).
%Many visually appealing and physically intricate phenomena are on this range of length scale. 
%Examples include the water-strider locomotion on fluid surface, chiral effects, xxx, and xxx.
%The underpinning physics behind these phenomena is xxx.

%% Motivation
%% 数值模拟这类现象的困难


%% Others' work

%% Challenges to solve

%% Contribution


%%%% related work

%%%% method

%%%% 1/22 进度
- 提纲已列在OneNote上
- Related Work

%%%% current problem: 1/22
- Table: 下标的规则是怎样定义的？
- shell全部改成membrane
- 方程1没有外力项？我建议完全参照Bush notes的2.1,2.2写, 粘性也写进方程里（不然不叫NS），然后再写我们实际求解的时候忽略了粘性
- 方程2讲的是数值离散，不需要
- 3.2讲的是数值离散，不需要放在这里
- Physical model里不能出现数值离散的模型!






